The Hidden Subsidy of the Affordable Care Act

Under the ACA, the federal government paid a substantially larger share of medical costs of newly eligible Medicaid enrollees than previously eligible ones. States could save up to 100% of their per-enrollee costs by reclassifying original enrollees into the newly eligible group. We examine whether this fiscal incentive changed states' enrollment practices. We find that Medicaid expansion caused large declines in the number of beneficiaries enrolled in the original Medicaid population, suggesting widespread reclassifications. In 2019 alone, this phenomenon affected 4.4 million Medicaid enrollees at a federal cost of $8.3 billion. Our results imply that reclassifications inflated the federal cost of Medicaid expansion by 18.2%.

==> Output_annual/results_12_7_2023_never.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{10}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}&\multicolumn{1}{c}{(10)}\\
            &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} \\
\hline
ATT         &     -0.0887\sym{**} &     -0.0654\sym{*}  &     -0.0914\sym{**} &     -0.0783\sym{*}  &     -0.0957\sym{**} &     -0.0586\sym{+}  &     -0.0838\sym{**} &     -0.0532         &                     &     -0.0639\sym{+}  \\
            &    (0.0286)         &    (0.0311)         &    (0.0287)         &    (0.0333)         &    (0.0371)         &    (0.0324)         &    (0.0318)         &    (0.0339)         &                     &    (0.0367)         \\
[1em]
simple      &                     &                     &                     &                     &                     &                     &                     &                     &     -0.0532         &                     \\
            &                     &                     &                     &                     &                     &                     &                     &                     &    (0.0357)         &                     \\
\hline
\(N\)       &         714         &         714         &         714         &         714         &         714         &         714         &         714         &         714         &         616         &         616         \\
\hline\hline
\multicolumn{11}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{11}{l}{\footnotesize \sym{+} \(p<0.10\), \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> Output_annual/results_12_7_2023_never_no_Wooldridge.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{9}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}\\
            &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} \\
\hline
ATT         &     -0.0887\sym{**} &     -0.0654\sym{*}  &     -0.0914\sym{**} &     -0.0783\sym{*}  &     -0.0957\sym{**} &     -0.0586\sym{+}  &     -0.0838\sym{**} &     -0.0532         &     -0.0639\sym{+}  \\
            &    (0.0286)         &    (0.0311)         &    (0.0287)         &    (0.0333)         &    (0.0371)         &    (0.0324)         &    (0.0318)         &    (0.0339)         &    (0.0367)         \\
\hline
\(N\)       &         714         &         714         &         714         &         714         &         714         &         714         &         714         &         714         &         616         \\
\hline\hline
\multicolumn{10}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{10}{l}{\footnotesize \sym{+} \(p<0.10\), \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}

